CILIATE: Towards Fairer Class-based Incremental Learning by Dataset and Training Refinement

Due to the model aging problem, Deep Neural Networks (DNNs) need updates to adjust them to new data distributions. The common practice leverages incremental learning (IL), e.g., Class-based Incremental Learning (CIL) that updates output labels, to update the model with new data and a limited number of old data. This avoids heavyweight training (from scratch) using conventional methods and saves storage space by reducing the number of old data to store. But it also leads to poor performance in fairness. In this paper, we show that CIL suffers both dataset and algorithm bias problems, and existing solutions can only partially solve the problem. We propose a novel framework, CILIATE, that fixes both dataset and algorithm bias in CIL. It features a novel differential analysis guided dataset and training refinement process that identifies unique and important samples overlooked by existing CIL and enforces the model to learn from them. Through this process, CILIATE improves the fairness of CIL by 17.03%, 22.46%, and 31.79% compared to state-of-the-art methods, iCaRL, BiC, and WA, respectively, based on our evaluation on three popular datasets and widely used ResNet models.

==> ack.tex <==
%!TEX root = paper.tex


==> trash/bg.tex <==
% Class-based IL learns from a stream of different categories of data batches, and aims to exploit knowledge from previous classes to improve learning of new ones, as well as exploiting new data to improve performance on previous ones~\cite{masanaClassincrementalLearningSurvey2020}.
% Class-based IL focuses on learning a sequence of tasks, where task refers to a set of classes disjoint from other~(previous or future) data's classes.
% Learners are allowed to process the training data of the current task multiple times during the training session. 
% Besides, class-based IL use a small memory to store some exemplars from previous tasks.

% More formally, given a model trained on $n$ old classes, with feeding $m$ new classes we get a new model to perform classification on $n+m$ classes.
% We call this process an \textit{incremental step}.
% Assume the total number of the samples in new classes ${X^m}=\left\{(x_i,y_i),1\leq i\leq M,y_i\in [n+1,\dots,n+m]\right\}$ and the selected exemplars from old classes $\hat{X}^n=\left\{(x_j,y_j),1\leq j\leq N_s,y_j\in [1,\dots,n]\right\}$ is $M$ and $N_s$, respectively.
% Then we denote the output as $\hat{\mathbf{o}}^n(x)=[\hat{o}_1(x),\dots,\hat{o}_n(x)]$ and $\mathbf{o}^{n+m}(x)=[\hat{o}_1(x),\dots,\hat{o}_{n+m}(x)]$ for the old and new model respectively.
% Following such notations, we can define the classification loss as:
% \begin{equation}
%     L_c=\sum_{(x,y)\in \hat{X}^n\cup X^m}\sum^{n+m}_{k=1}-t_k\log{[p_k(x)]}
%     \label{eq:CEloss}
% \end{equation}
% where $t_k$ is the truth label and $p_k(x)$ is the output probability of the $k$-th class in total $n+m$ classes.

% The distillation loss is often combined with classification loss, which can be formulated as follows:
% \begin{equation}
%     \begin{aligned}
%         L_k = \sum_{(x,y)\in \hat{X}^n\cup X^m}\sum^{n+m}_{k=1}-\hat{\pi}_k(x)\log{[\pi_k(x)]}\\
%         \hat{\pi}_k(x)=\frac{e^{\hat{o}_k(x)/T}}{\sum^n_{j=1}e^{\hat{o}_j(x)/T}},
%         \pi_k(x)=\frac{e^{o_k(x)/T}}{\sum^n_{j=1}e^{o_j(x)/T}}
%     \end{aligned}
%     \label{eq:KDloss}
% \end{equation}
% where $T$ is the temperature scalar. So we can define the combined loss containing two terms as:


% \smallskip
% \noindent \textbf{Memory restrictions.}
% Some systems, such as mobile applications and embedded systems, have physical limitations for storage memory, so they cannot simply store all seen data and perform the joint training strategies.
% IL only require processing of new data when updating the system, which reduces the memory footprint significantly.

% \smallskip
% \noindent \textbf{Data security \& privacy.}
% Security and privacy considerations are common in legislation-related systems such as health applications.
% IL prevents the long-term and centralized storage of sensitive data from users.

% \smallskip
% \noindent \textbf{Time \& energy consumption.}
% The overhead of training deep neural network can be exorbitant.
% The time cost and carbon footprint of retraining systems for every new data update is considerable, which will even grow in the coming years~\cite{sharirCostTrainingNlp2020,masanaClassincrementalLearningSurvey2020}.
% IL provides a more computationally efficient way to update a system.

